Uniformly Area Expanding Flows in Spacetimes

The central object of study of this thesis is inverse mean curvature vector flow of two-dimensional surfaces in four-dimensional spacetimes. Being a system of forward-backward parabolic PDEs, inverse mean curvature vector flow equation lacks a general existence theory. Our main contribution is proving that there exist infinitely many spacetimes, not necessarily spherically symmetric or static, that admit smooth global solutions to inverse mean curvature vector flow. Prior to our work, such solutions were only known in spherically symmetric and static spacetimes. The technique used in this thesis might be important to prove the Spacetime Penrose Conjecture, which remains open today. Given a spacetime $(N^{4}, \overline{g})$ and a spacelike hypersurface $M$. For any closed surface $\Sigma$ embedded in $M$ satisfying some natural conditions, one can "steer" the spacetime metric $\overline{g}$ such that the mean curvature vector field of $\Sigma$ becomes tangential to $M$ while keeping the induced metric on $M$. This can be used to construct more examples of smooth solutions to inverse mean curvature vector flow from smooth solutions to inverse mean curvature flow in a spacelike hypersurface.

==> Abbreviations/listofabbr.tex <==
\abbreviations

% You can put here what you like, but here's an example
%Note the use of starred section commands here to produce proper division
%headers without bad '0.1' numbers or entries into the Table of Contents.
%Using the {\verb \begin{symbollist} } environment ensures that entries are
%properly spaced.

\section*{Symbols}

Put general notes about symbol usage in text here.  Notice this text is
double-spaced, as required.

\begin{symbollist}
	\item[$\mathbb{X}$] A blackboard bold $X$.  Neat.
	% Optional item argument makes the symbol/abbr
	\item[$\mathcal{X}$] A caligraphic $X$.  Neat.
	\item[$\mathfrak{X}$] A fraktur $X$.  Neat.
	\item[$\mathbf{X}$] A boldface $X$.
	\item[$\mathsf{X}$] A sans-serif $X$. Bad notation.
	\item[$\mathrm{X}$] A roman $X$.
\end{symbollist}

\section*{Abbreviations}

Long lines in the \texttt{symbollist} environment are single spaced, like in
the other front matter tables.

\begin{symbollist}
	\item[AR] Aqua Regia, also known as hydrocloric acid plus a splash of 
	nitric acid.
	\item[SHORT] Notice the change in alignment caused by the label width
	between this list and the one above.  Also notice that this multiline
	description is properly spaced. 
	\item[OMFGTXTMSG4ME] Abbreviations/Symbols in the item are limited to
	about a quarter of the textwidth, so don't pack too much in there.
	You'll bust the margins and it looks really bad.
\end{symbollist}

==> Chapter4/imcvf_backup.tex <==
\chapter{Inverse Mean Curvature Vector Flow}
\label{chap:imcvf}

In this chapter we study the central object in this thesis: \emph{inverse mean vector curvature flow} (IMCVF) of codimension two surfaces in a spacetime. Surfaces we study here satisfy the topological and geometric setups defined in Section \ref{sec:codim two surface geometry}. In Section \ref{sec:motivation for imcvf} we recall the definition of IMCVF and the geometric obstruction for bad existence theory of such flows. Then we use IMCVF in spherically symmetry and the Huisken-Ilmanen IMCF as motivations for finding spacetimes in which IMCVFs of surfaces exist.  In Section \ref{sec:construction of imcvf coordinates} we construct a spacetime with a set of coordinates from scratch, just as we did in the spherically symmetric case. We then prove that there exist infinitely many spacetime metrics such that IMCVF exists, and hence IMCVF in fact exists generically. In Section \ref{sec:coordinate free description of imcvf and steering parameters} we give a coordinate-free description of IMCVF using steering parameters. Finally in Section \ref{sec:generalizations of imcvf} we discuss some generalizations of the technique we use in constructing IMCVF coordinates. 

\section{Motivations from Spherically Symmetric Spacetimes and Huisken-Ilmanen IMCF}
\label{sec:motivation for imcvf}
Given a spacetime $(N^{4}, \gbar)$ and a closed codimension two surface $\Sigma$ with induced metric $g_{\Sigma}$ and mean curvature vector $\vec{H}_{\Sigma}$, recall from Section \ref{subsec:mean curvature vector, hawking mass, normal variation} that a \emph{smooth inverse mean curvature vector flow} (IMCVF) of $\Sigma$ is a normal variation 
\[F: \Sigma \times [0, T]\longrightarrow N, \quad (\Sigma, s)\mapsto F(\Sigma, s) =: \Sigma_{s},\] 
such that 
\begin{equation}\label{equ:IMCVF equation revisit}
\frac{\p}{\p s}F(x, s) = \vec{I}_{\Sigma_{s}}(x, s),\quad \forall\, (x, s)\in \Sigma_{s},
\end{equation}
where $\vec{I}_{\Sigma_{s}}$ is the inverse mean curvature vector of $\Sigma_{s}$ defined as
\[\vec{I}_{\Sigma_{s}}: = -\frac{\vec{H}_{\Sigma_{s}}}{\<\vec{H}_{\Sigma_{s}}, \vec{H}_{\Sigma_{s}}\>_{\gbar}}.\]
The IMCVF equation \ref{equ:IMCVF equation revisit} (same as Equation \ref{equ:IMCVF equation}) is a forward-backward (or reverse) parabolic PDE, hence lacks a general existence theory. For instance the \emph{reverse heat flow} equation is a forward-backward parabolic equation. Since the \emph{forward heat flow} equation smooths out instantaneously once the flow starts, the reverse heat flow in general develops singularity instantaneously. However as we remarked in the introduction, the reverse heat flow exists for time $T > 0$ if  we first perform the forward heat flow for time $T$ and then flow backwards. The point is that even forward-backward parabolic PDEs in general do not have good existence theory, such PDEs can still be solvable if we start with the ``right'' initial condition (e.g. in reverse heat flow, we start with where forward heat flow stops). However this notion of a ``right'' initial condition is quite ambiguous, and can be quite hard to guess in the case of IMCVF. 

Another idea is to pick any reasonable initial condition to start the flow, and then controls the path of the flow so that singularities can be avoided. For instance, IMCVF of spheres exist in spherically symmetric spacetimes. This is due to the mean curvature vector computation in Equation \ref{equ:mean curvature of sphere in spherically symmetric spacetime} in spherical symmetry: it is radial and has no components in the timelike direction, therefore the IMCVF of spheres will be contained inside $t = \text{constant}$ spacelike slices. Geometrically, spherical symmetry eliminates all the ``time wiggles'' of the flow surfaces, hence restricting the flow direction to be spacelike. Since the IMCVF equation is forward-backward parabolic only in the timelike direction, IMCVF exists without running into singularities in spherical symmetry (see Figure \ref{fig:foliation of spherically symmetric spacetime with spheres in IMCVF}).

How do we generalize the spherically symmetric case to general spacetimes? Note that the mean curvature vector $\vec{H}_{\Sigma}$ of $\Sigma$ is a section of the normal bundle $N\Sigma$, thus has a timelike component and a spacelike component. Motivated by the spherically symmetric case, intuitively if the flow surfaces all have purely \emph{spacelike} mean curvature vectors, we might hope to get a better existence theory. The following proposition confirms this intuition:

\begin{proposition}\label{prop:spacelike IMCVF equals tangential mean curvature in IMCF}
The family of closed embedded surfaces $\{\Sigma_{s}\}$ is a solution to the smooth IMCVF with \emph{spacelike} inverse mean curvature vector $\vec{I}_{\Sigma_{s}}$ everywhere on the surfaces if and only if there exists a spacelike hypersurface $M^{3}\subset N$, such that the mean curvature vector $\vec{H}_{\Sigma_{s}}$ is tangential to $M$ at all $(x, s)$, and $\{\Sigma_{s}\}$ is a solution to the smooth Huisken-Ilmanen IMCF in $M$.
\end{proposition}

\begin{proof}
Given $\{\Sigma_{s}\}$ a solution to the smooth \emph{spacelike} IMCVF. Consider the hypersurface $M$ of $N$ defined by the union of all the surfaces $\Sigma_{s}$, i.e. the ``sweep out'' region of the the flow surfaces. Since the flow is smooth and spacelike, $M$ is a smooth manifold which is spacelike as well. Now $\vec{H}_{\Sigma_{s}}$ is tangential to $M$ by the construction of $M$. Since $\Sigma_{s}$ is of codimension one in $M$, $\vec{H}_{\Sigma_{s}}$ is parallel to the unit outward normal vector field $\nu_{\Sigma_{s}}$ along $\Sigma_{s}$, i.e.,
\begin{equation}
\vec{H}_{\Sigma_{s}} = -\lambda \nu_{\Sigma_{s}},
\end{equation}
at each $(x, s)\in \Sigma_{s}$ for some smooth positive function $\lambda$. $\lambda$ is chosen to positive since $\vec{H}_{\Sigma_{s}}$ points in the inward normal direction. Therefore
\begin{equation}\label{spacelike IMCVF implies IMCF}
\vec{I}_{\Sigma_{s}} = -\frac{\vec{H}_{\Sigma_{s}}}{\<\vec{H}_{\Sigma_{s}}, \vec{H}_{\Sigma_{s}}\>_{\gbar}} = \frac{\lambda \nu_{\Sigma_{s}}}{\<-\lambda \nu_{\Sigma_{s}}, -\lambda \nu_{\Sigma_{s}}\>} = \frac{\lambda \nu_{\Sigma_{s}}}{\lambda^{2} \<\nu_{\Sigma_{s}}, \nu_{\Sigma_{s}}\>} = \frac{\nu_{\Sigma_{s}}}{\lambda} = \frac{\nu_{\Sigma_{s}}}{H_{\Sigma_{s}}},
\end{equation}
where $H_{\Sigma_{s}}$ is the mean curvature scalar of $\Sigma_{s}$ in the direction of $\nu_{\Sigma_{s}}$, defined by Equation \ref{def:mean curvature scalar}:
\begin{equation*}
H_{\Sigma_{s}} : = -\<\vec{H}_{\Sigma_{s}}, \nu_{\Sigma_{s}}\> = -\<-\lambda \nu_{\Sigma_{s}}, \nu_{\Sigma_{s}}\> = \lambda.
\end{equation*}
Thus in particular $H_{\Sigma_{s}} > 0$. From equation (\ref{spacelike IMCVF implies IMCF}), we see that $\{\Sigma_{s}\}$ indeed is a solution to the smooth IMCF in $M$.
\\
Conversely, suppose $M$ is a spacelike hypersurface and $\{\Sigma_{s}\}$ is a solution to the smooth IMCF in $M$. Assuming that $\vec{H}_{\Sigma_{s}}$ is tangential to $M$ at each $(x, s)$, we know that $\vec{H}_{\Sigma_{s}}$ is spacelike as well. Moreover, by the same computation as in equation ($\ref{spacelike IMCVF implies IMCF}$), we have 
\[\frac{\nu}{H}_{\Sigma_{s}} = \vec{I}_{\Sigma_{s}}.\]
Thus $\{\Sigma_{s}\}$ is a solution to the smooth IMCVF in $N$, with spacelike mean curvature vectors.
\end{proof}

Therefore spacelike smooth IMCVF in $N$ is equivalent to smooth Huisken-Ilmanen IMCF in a spacelike hypersurface of $N$. This suggests that instead of looking for solutions to the smooth IMCVF solutions, we can study:

\begin{mydef}[Smooth (resp. Weak) Spacelike IMCVF] \label{def:spacelike IMCVF}
A smooth (resp. weak) \emph{spacelike} IMCVF of $\Sigma$ is a smooth IMCVF $F: \Sigma \times [0, T]\longrightarrow N$ of $\Sigma$ such that there exists a spacelike hypersurface $M$ of $N$ containing $F(\Sigma, s)$, for all $s\in [0, T]$, moreover $\vec{H}_{\Sigma_{s}}$ is tangential to $M$ everywhere, and $F$ is a smooth (resp. weak) Huisken-Ilmanen IMCF in $M$. Here weak Huisken-Ilmanen IMCF refers to IMCF with jumps. 
\end{mydef}

Now the questions are: 
\begin{itemize}
\item Given a spacetime and a surface $\Sigma$, what is this spacelike slice $M$ in which we perform Huisken-Ilmanen IMCF of $\Sigma$? 
\item Moreover, given a surface $\Sigma$ and a spacelike slice $M$ containing $\Sigma$, how do we ``steer'' its IMCVF flow path of $\Sigma$ so that it stays inside $M$ (i.e. maintaining tangential flow direction)? 
\end{itemize}
To answer these questions, we first assume that these questions have positive answers: suppose our spacetime $N$ is foliated by spacelike slices, and for any such slice $M$, it is foliated by Huisken-Ilmanen IMCF of topological two-spheres, then we can parameterize $N$ using four parameters: two parameters describe the topological two-spheres, one describes which sphere we are on inside a fixed slice, and the remaining one describes which spacelike slice we are on. Conversely if we can find a spacetime with a special set of coordinates, such that the coordinates are results of this particular foliation, then the spacelike IMCVF of the topological two-spheres exists in this spacetime. Now the question is: What exactly are the conditions that this set of coordinates should satisfy? And do such coordinates exist? We study these two questions in the following section, and we answer the latter in the affirmative.

\section{Construction of Spacelike IMCVF Coordinates}
\label{sec:construction of imcvf coordinates}
\subsection{Parameterizing the Spacetime Using Foliations Coordinates}
We will assume that our spacetime $(N^{4}, \gbar)$ is topologically equivalent to $\RR^{4}$ (i.e. with no blackholes) for the remaining of this chapter. We study parameterizations of $N$ using coordinates that results of foliations in the spacetime, called \emph{foliation coordinates}. We start with a rather general foliation, motivated by the spherically symmetric case (as in Figure \ref{fig:foliation of spherically symmetric spacetime with spheres in IMCVF}). 

First of all pick any topological cylinder $D^{3} \times \RR$ inside the spacetime $N$, where $D^{3}$ is the three-dimensional disk with boundary two-spheres. Then we pick an arbitrary slicing of the cylinder using three-dimensional spacelike hypersurfaces, and this slicing \emph{defines} the $t$ coordinate: we define each slice as $t = \text{constant}$.  This is the coordinate that tells us which hypersurface slice we are on in the spacetime. 

Next given a particular slice $M$, the intersection of $M$ with the cylinder is a topological two-sphere, denoted as $S$. We parametrize $S$ using arbitrary coordinate functions $\{\theta, \phi\}$. Now pick an arbitrary variation of $S$ that foliates the slice $M$ (except a point, but this is fine with our study), and the variational vector field defines the last coordinate $r$ that tells us which of the variational surfaces we are on inside $M$.

Now we have constructed the general foliation coordinates $\{t, r, \theta, \phi\}$, and the spacetime metric $\gbar$ has the following corresponding coordinate representations:



As a new set of coordinates of the spacetime we get to specify four conditions on them (since the $N$ is four-dimensional, a change of coordinates is given by four functions). The first condition is requiring the flow of the two-spheres in each slice $M$ to be in the normal direction, since IMCVF is a normal flow. This corresponds to requiring
\[\<\ppr, \pptheta\>_{\gbar} = 0, \quad \<\ppr, \ppphi\>_{\gbar} = 0.\]
$\ppr$ is called the radius direction of flows of spheres, analogous to the radial flow of spheres in spherically symmetric spacetimes.

Next we want the coordinate topological sphere $S_{t,r}$ at slice $t$ and ``radius''
\subsection{Mean Curvature Vector of $S_{t,r}$}
\label{subsec:mean curvature of coordinate sphere}

\subsection{Condition of Mean Curvature Vector Being Radial}
\label{subsec:radial mean curvature vector condition}

\section{Coordinate Free Description and Steering Parameters}
\label{sec:coordinate free description of imcvf and steering parameters}


\section{Generalizations}
\label{sec:generalizations of imcvf}

==> Chapter6/timeflatsurface.tex <==
\chapter{Time Flat Surfaces}
\label{chap:timeflatsurface}

In this chapter, we briefly discuss time-flat surfaces, first defined by H. Bray, J. Jauregui and M. Mars \cite{BrayJauregui2014}. 

\begin{mydef}[Uniformly Area Expanding Flows]\label{def:uniformly area expanding flow}
Given a spacetime $(N^{4}, \gbar)$ and a codimension-two closed embedded surface $\Sigma^{2}$. A \emph{uniformly area expanding flow} of $\Sigma$ is a normal variation $F:\Sigma \times [0, T] \longrightarrow N$ such that
\begin{equation}\label{equ:uniformly area expanding flow direction}
\frac{\p}{\p s}F(x, s) = \vec{\xi} = \vec{I_{s}} + \beta \vec{I_{s}}^{\perp}, \quad s\in [0, T].
\end{equation}
where $\beta\in C^{\infty}(N)$, and $\vec{I}_{s}$ is the inverse mean curvature vector of the flow surface $\Sigma_{s}: = F(\Sigma, s)$.
\end{mydef}

With this definition, IMCVF is an area expanding flow with $\beta = 0$ in (\ref{def:uniformly area expanding flow}). A natural question is whether the Hawking mass is monotone under general area expanding flows. However, H. Bray, J. Jauregui and M. Mars have recently shown that this isn't true in general:

\begin{theorem}[\cite{BrayJauregui2014}]\label{thm:variation of Hawking mass under uniformly area expanding flow}
Given a uniformly area expanding family of surfaces $\Sigma_{s}$, we have
\begin{align*}
\frac{\frac{d}{ds}m_{H}(\Sigma_{s})}{\sqrt{\frac{|\Sigma_{s}|}{(16\pi)^{2}}}} & = 4\pi (2 - \chi(\Sigma_{s})) + \int_{\Sigma_{s}}2G(-\vec{H}_{s}^{\perp}, \vec{\xi}^{\perp}) \\
& + \int_{\Sigma_{s}}\left[|\mathring{\II_{r}}|^{2} + 2\beta\<\mathring{\II_{r}}, \mathring{\II_{t}}\> + |\mathring{\II_{t}}|^{2} \right] \\
& + \int_{\Sigma_{s}}2\left[ \left|\frac{\na_{\Sigma}H_{s}}{H_{s}} + 2\beta \alpha_{H}\left(\frac{\na_{\Sigma} H}{H}  + |\alpha_{H}|^{2} \right) \right|^{2} \right]\\
& + \int_{\Sigma_{s}}2\beta \cdot \divg_{\Sigma_{s}}(\alpha_{H}),
\end{align*}
where $G$ is the Einstein curvature tensor, $\II_{r} = -\<\vec{\II}, \nu_{H}\>$ and $\II_{t} = -\<\vec{II}, \nu_{H^{\perp}}\>$ are the scalar-valued components of the second fundamental form $\vec{\II}$; $\mathring{\II_{r}}$ and $\mathring{\II_{t}}$ are the tracefree parts of $\II_{r}$ and $\II_{t}$, respectively; $H_{s} = |\vec{H}_{s}|$ is the length of the mean curvature vector of $\Sigma_{s}$, and $\alpha_{H}$ is the connection one-form associated with $\nu_{H} = -\frac{\vec{H}}{|\vec{H}|}$.
\end{theorem}

The first term is non-negative since $\chi(\Sigma_{s}) \leq 2$. The next three terms in (\ref{thm:variation of Hawking mass under uniformly area expanding flow}) are non-negative if the spacetime satisfies the dominant energy condition is satisfied, $-1 \leq \beta \leq 1$ and the mean curvature vector of each flow surface is inward-spacelike. Therefore, the Hawking mass is monotone under uniformly area expanding flows if and only if
\begin{equation}\label{equ:critical term in the variation of Hawking mass under uniformly area expanding flow}
\int_{\Sigma_{s}}2\beta \cdot \divg_{\Sigma_{s}}(\alpha_{H}) \geq 0.
\end{equation}

Notice that if $\beta = 0$ (IMCVF) or $\beta$ is constant on each flow surface $\Sigma_{s}$ (discussed in Chapter \ref{chap:imcvf}), then (\ref{equ:critical term in the variation of Hawking mass under uniformly area expanding flow}) vanishes, and hence we get the desired monotonicity. For a general smooth function $\beta$, if 
\begin{equation}\label{equ:time flat condition}
\divg_{\Sigma_{s}}(\alpha_{H}) = 0,
\end{equation}
then (\ref{equ:critical term in the variation of Hawking mass under uniformly area expanding flow}) vanishes as well. 

\begin{mydef}[\cite{BrayJauregui2014}]\label{def:time flat surface}
A surface $\Sigma$ is called \emph{time flat} if $\divg_{\Sigma_{s}}(\alpha_{H}) = 0$.
\end{mydef}

Using this the following theorem can be proved:

\begin{theorem}[\cite{BrayJauregui2014}]
For a uniformly area expanding family of connected time flat surfaces flowing in spacelike directions in a spacetime satisfying the dominant energy condition,
\[\frac{d}{ds}m_{H}(\Sigma_{s}) \geq 0.\]
\end{theorem}
